Sharp Nonuniqueness in the Transport Equation with Sobolev Velocity Field

Given a divergence-free vector field ${\bf u} \in L^\infty_t W^{1,p}_x(\mathbb R^d)$ and a nonnegative initial datum $\rho_0 \in L^r$, the celebrated DiPerna--Lions theory established the uniqueness of the weak solution in the class of $L^\infty_t L^r_x$ densities for $\frac{1}{p} + \frac{1}{r} \leq 1$. This range was later improved in [BCDL21] to $\frac{1}{p} + \frac{d-1}{dr} \leq 1$. We prove that this range is sharp by providing a counterexample to uniqueness when $\frac{1}{p} + \frac{d-1}{dr} > 1$. To this end, we introduce a novel flow mechanism. It is not based on convex integration, which has provided a non-optimal result in this context, nor on purely self-similar techniques, but shares features of both, such as a local (discrete) self similar nature and an intermittent space-frequency localization.

==> To_be_discraded.tex <==
%March 17: Added by Anuj
%March 17: Added by Anuj
%March 17: Added by Anuj
%March 17: Added by Anuj
{\color{red}
\section{Fundamental aspects of the  construction}
\label{sec: nonunique measure}


To introduce the fundamental aspects of our construction, we begin by briefly outlining the work of the third author \cite{kumar2023nonuniqueness}, which served as our starting point. The main result of \cite{kumar2023nonuniqueness} was to build an explicit example of a divergence-free vector field 
\begin{equation}
    \bs{u} \in C([0, 1]; W^{1, p}(\R^d;\R^d) \cap C^\alpha([0,1] \times \R^d) \, , \quad \text{for a given $p<d$ and $\alpha\in (0,1)$}
\end{equation}
and an associated flow map $X_{\bs{u}}$ that
maps the whole domain to a Cantor set $\mathcal{C}_\Phi$ whose Hausdorff dimension is $s<d$ at $t = 1$. 


\bigskip

As a corollary, it follows that set of initial condition
for which the trajectories of $\bs{u}$ are not unique is of full Lebesgue measure. Indeed, from \cite{DiPernaLions,Ambrosio04} we know that a Regular Lagrangian flow associated to $\bs{u}$ exists. However, the latter must be measure preserving hence it does not coincide with $X_{\bs{u}}$ on a set of full measure.



\bigskip

To constructs $\bs{u}$, \cite{kumar2023nonuniqueness} builds a vector field
\begin{equation}
    \bs{v} \in C^\infty([0,1) \times \R^d) \cap C([0, 1]; W^{1, p}(\R^d;\R^d) \cap C^\alpha([0,1] \times \R^d)
\end{equation}
whose associated flow $X_{\bs{v}}$ is well defined and unique for every $x\in \R^d$  $\forall \; 0\le t \le 1$. Moreover, $X_{\bs{v}}$ maps the Cantor set $\mathcal{C}_\Phi$ to the uniform distribution at time $t=1$.
The vector field $\bs{u}$ and the flow map $X_{\bs{u}}$ is obtained by time-reversing $\bs{v}$ and the associated flow map $X_{\bs{v}}$.

\bigskip

\begin{figure}[h]
\centering
 \includegraphics[scale = 0.5]{Figures/ODE_paper.eps}
 \caption{is adapted from \cite{kumar2022three}. The figure shows a few steps of how the vector field $\bs{v}$ distribute points in the Cantor set to the whole domain.}
 \label{fig: ODE paper}
 \end{figure}

\bigskip



The vector field $\bs{v}$ acts in infinite number of consecutive steps, where the $i$th step takes place over a time span of  $\frac{T_0}{2^{\beta i} }$ for some constants $T_0$, $0<\beta<1$.  In the $i$th step, the function of the vector field $\bs{v}$ is to translate the $i$th generation cubes in the Cantor set process so that their center is aligned with $i$th generation dyadic cube. The first four steps of this construction are shown in Figure \ref{fig: ODE paper}. The size of cubes translated at the $i$th stage by this vector field $\bs{v}$ is much smaller than the $i$th generation dyadic cubes and is the key reason for the control on the Sobolev norm of $\bs{v}$.


Finally, at the end of infinite steps the points in the Cantor set $\mathcal{C}_{\Phi}$ is distributed to the whole domain in finite time. We refer the reader to \cite[Section 3]{kumar2023nonuniqueness} for a complete overview of the construction of the vector field $\bs{v}$. 


\bigskip

In constructing $\bs{v}$, \cite{kumar2023nonuniqueness}, employed a divergence-free vector field ``blob flow'' to rigidly translate a cube without deformation. The same blob flow is utilized in our construction of nonunique $L^r$ solutions to the transport equation as well. We provide the details of this flow, along with some minor modifications, in Section \ref{sec: building block}.




\subsection{Measure valued solutions}

The vector field $\bs{v}\in C([0,1]; W^{1,p}(\mathbb{T}^d, \mathbb{R}^d))$ can be used to produce nonunique measure-valued-solutions to the continuity equation since the flow map $X_{\bs{v}}$ satisfies
\begin{equation}
    X_{\bs{v}}(t,\cdot)_{\#} c\mathcal{H}^s|_{\mathcal{C}_\Phi} \to \mathscr{L}^d|_{[-1/2,1/2]^d} \, , \quad \text{as $t\to 1$}\, ,
\end{equation}
in the weak star topology, where $c$ is a scaling constant that makes the left hand side a probability measure. This easily implies that the continuity equation associated with $\bs{u}$ admits two distinct measure-valued solutions with initial condition $\mathscr{L}^d|_{[-1/2,1/2]^d}$.


\subsection{Beyond measure-valued solutions}


The example in \cite{kumar2023nonuniqueness}, as outlined above, does not produce nonuniqueness in the class of densities $\rho \in L^\infty([0,1];L^r)$ for any $r \geq 1$. The density solution corresponding to the vector field $\bs{u}$ (time-reversed version of $\bs{v}$) immediately becomes measure anytime after $t=0$. One of the main challenge to construct nonunique $L^r$ solutions is to avoid immediate concentration of the density field. To overcome this challenge and to sharply match with the uniqueness range found in \cite{BrueColomboDeLellis21}, we introduce a new construction based on two novel ideas:


\begin{enumerate}[label = (\arabic*)]
    \item \underline{Interweaving the scaled copies of the vector field within itself:} We construct a vector field $\bs{v}$, which consists of infinite number of steps, as in \cite{kumar2023nonuniqueness}. However, in between the $i$th and $i+1$th step, we appropriately interweave spatially- and temporally-scaled copies of the vector field $\bs{v}$ itself. This first idea is presented in Section \ref{sec: p=1} and allows us to prove nonuniqueness in the class of densities $\rho\in L^\infty([0,1];L^1)$, but no better.


    
    \item \underline{Asynchronous translation of cubes:}
    To extend beyond $L^1$ integrability of densities, we introduce asynchronous motion of cubes in constructing the vector field $\bs{v}$. This renders $\bs{v}$ spatially heterogeneous compared to the constructions in \cite{kumar2023nonuniqueness} and our $L^1$ case. The construction of this vector field is given in Section \ref{sec: outline} and allows us to cover a range of exponents beyond what is available using the method of convex integration and match with the range for the uniqueness of solutions given in \cite{BrueColomboDeLellis21}.
\end{enumerate}

% {\color{blue}
% EB: We should mention (without many details):
% \begin{itemize}
%     \item Blob vector fields 
%     \item Explanation of non-uniqueness of trajectories
% \end{itemize}
% It would be nice to add have some of the pictures in \cite{kumar2023nonuniqueness} to explain the action of the vector field.
% }

% {\color{violet}AK: Does this subection now look good?}



}

==> contraction.tex <==
\section{Proof of contraction}
\label{sec: contraction}
In this section, we show that the mappings $F$ and $G$ as defined in \S \ref{sec: fixed-point mapping} are contraction. We first focus on the mapping $F$ and define a set $\mathcal{X}$ of infinite sequences of vector fields as
\begin{align}
\mathcal{X} \coloneqq \Bigg\{ \{\bs{w}_i\}_{i \in \mathbb{N}} \in \ell^\infty_{\gamma_1}\left(\mathbb{N}; C([0, 1]; W^{1, p}(\mathbb{R}^d, \mathbb{R}^d))\right)  \; \Bigg| \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \nonumber \\
\nabla \cdot \bs{w}_i \equiv 0, \; \bs{w}_i(0, \cdot) = \bs{w}_i(1, \cdot) \equiv \bs{0},  \; \supp_{\bs{x}} \bs{w}_i(t, \cdot) \subseteq \left[-\frac{1}{2}, \frac{1}{2}\right]^d \Bigg\},
\end{align}
equip with a metric $\norm{\cdot}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}$. Our next goal is to show $F : \mathcal{X} \to \mathcal{X}$ is a contraction. As a first step, we show that the mapping $F$ defined on $\mathcal{X}$ takes values in $\mathcal{X}$. In the second step, we will show that the mapping defined on $\mathcal{X}$ is a contraction. \\
\\
Step 1 ($F: \mathcal{X} \to \mathcal{X}$): Let $\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}} \in \mathcal{X}$, then from the definition of $F$ in \S \ref{sec: fixed-point mapping} it is clear that for any $i \in \mathbb{N}$, we have
\begin{align}
\nabla \cdot F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}}) \equiv 0, \quad F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(0, \cdot) = F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(1, \cdot) \equiv \bs{0} \quad \nonumber \\
\text{and} \quad \supp_{\bs{x}} F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) \subseteq \left[-\frac{1}{2}, \frac{1}{2}\right]^d.
\end{align}
For $k \in \{1, \dots 2^{\eta d}\}$, if $t \in \mathcal{T}^k_{(1)}$, then a straightforward calculation gives
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}} \leq \frac{1}{\tau^k_{mid} - \tau^k_1} \left(\frac{1}{2^{\eta + \nu i}}\right)^{\frac{d}{p}} \norm{\bs{w}_1}_{C^\infty_t W^{1, p}_{\bs{x}}}, \nonumber \\
\leq \frac{2^{\gamma_1}}{\tau^k_{mid} - \tau^k_1} \left(\frac{1}{2^{\eta + \nu i}}\right)^{\frac{d}{p}} \norm{\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}.
\label{contraction: Fi est Tau 1}
\end{align}
If $t \in \mathcal{T}^k_{(2)}$, then we get
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}} \leq \frac{1}{\tau^k_{2} - \tau^k_{mid}} \left( \frac{1}{2^{\eta}}\right)^{\frac{d}{p}} \norm{\ol{\bs{v}}_b}_{C^\infty_t W^{1, p}_{\bs{x}}}, \nonumber \\
\lesssim \frac{1}{\vartheta^2} \frac{1}{\tau^k_{2} - \tau^k_{mid}} \left(\frac{1}{2^{2\eta + \nu(i+1)}}\right)^{\frac{d}{p} - 1}.
\label{contraction: Fi est Tau 2}
\end{align}
If $t \in \mathcal{T}^k_{(3)}$, then we get
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}} \leq \frac{1}{\tau^k_{\infty} - \tau^k_2} 
\left(\frac{1}{2^{\eta}}\right)^{\frac{d}{p}} \norm{\bs{w}_{i+1}}_{C^\infty_t W^{1, p}_{\bs{x}}}, \nonumber \\
\leq \frac{2^{\gamma_1(i+1)}}{\tau^k_{\infty} - \tau^k_2} 
\left(\frac{1}{2^{\eta}}\right)^{\frac{d}{p}} \norm{\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}.
\label{contraction: Fi est Tau 3}
\end{align}
Finally, for $t = \tau^{2^{\eta d}}_{\infty}$, we have
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}}  = 0.
\label{contraction: Fi est Tau 4}
\end{align}
From the definition of $F_i$ in \S \ref{sec: fixed-point mapping}, the continuity of the Sobolev norm $\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}}$ in time is clear in the interiors of $\mathcal{T}^k_{(1)}$, $\mathcal{T}^k_{(2)}$ and $\mathcal{T}^k_{(3)}$. Now combining the definition of $F_i$ with the information that $\bs{w}_i(0, \cdot) = \bs{w}_i(1, \cdot) \equiv \bs{0}$ and $\supp_t \ol{\bs{v}}_b \subseteq \left[\frac{1}{3}, \frac{2}{3}\right]$, we obtain the continuity of the Sobolev norm on the interfaces $\tau^k_1$, $\tau^k_{mid}$, $\tau^k_{2}$ and $\tau^k_{\infty}$.

Finally, noting estimates (\ref{contraction: Fi est Tau 1}), (\ref{contraction: Fi est Tau 2}), (\ref{contraction: Fi est Tau 3}) and (\ref{contraction: Fi est Tau 4}) and the continuity of the Sobolev norm in time gives
\begin{align}
& \frac{1}{2^{\gamma_1 i}} \norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})}_{C^\infty_t W^{1, p}_{\bs{x}}} \lesssim_{\beta, \eta, \nu}  \nonumber \\ 
& \qquad \qquad  \sup_{i \in \mathbb{N}} \; \max\left\{\frac{1}{2^{\gamma_1 i}} \left(\frac{1}{2^{\nu i}}\right)^{\frac{d}{p}},  \frac{1}{2^{\gamma_1 i}} \left(\frac{1}{2^{\nu i}}\right)^{\frac{d}{p} - 1}\right\} \max\left\{1, \norm{\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}\right\}.
\end{align}
Therefore, the required condition for $F(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}}) \in \mathcal{X}$ is
\begin{align}
\gamma_1 \geq \nu\left(1 - \frac{d}{p}\right).
\label{contraction: F cond 1}
\end{align}
\noindent
Step 2 ($F$ \textit{is a contraction}): In  a way similar to Step 1, one finds that if $t \in \mathcal{T}^k_{(1)}$ then we get
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - F_i(\{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}} 
\leq 
\frac{2^{\gamma_1}}{\tau^k_{mid} - \tau^k_1} \left(\frac{1}{2^{\eta + \nu i}}\right)^{\frac{d}{p}} \norm{\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}} - \{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}.
\label{contraction: diff Fi est Tau 1}
\end{align}
If $t \in \mathcal{T}^k_{(2)}$ then we get
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - F_i(\{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}}  = 0.
\label{contraction: diff Fi est Tau 2}
\end{align}
If $t \in \mathcal{T}^k_{(3)}$ then we get
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - F_i(\{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}} 
\leq 
\frac{2^{\gamma_1(i+1)}}{\tau^k_{\infty} - \tau^k_2} 
\left(\frac{1}{2^{\eta}}\right)^{\frac{d}{p}} \norm{\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}} - \{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}.
\label{contraction: diff Fi est Tau 3}
\end{align}
If $t = \tau^{2^{\eta d}}_{\infty}$ then we get
\begin{align}
\norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - F_i(\{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{W^{1, p}}  = 0.
\label{contraction: diff Fi est Tau 4}
\end{align}
Combining everything above gives
\begin{align}
& \frac{1}{2^{\gamma_1 i}} \norm{F_i(\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}}) - F_i(\{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}})}_{C_t W_{\bs{x}}^{1, p}} \leq \nonumber \\
& \qquad \qquad  \sup_{i \in \mathbb{N}} \max \left\{\frac{2^{\gamma_1}}{\tau^k_{mid} - \tau^k_1} \frac{1}{2^{\gamma_1 i}} \left(\frac{1}{2^{\eta + \nu i}}\right)^{\frac{d}{p}}, \frac{2^{\gamma_1}}{\tau^k_{\infty} - \tau^k_2} 
\left(\frac{1}{2^{\eta}}\right)^{\frac{d}{p}}\right\} \norm{\{\bs{w}_{i^\prime}\}_{i^\prime \in \mathbb{N}} - \{\wt{\bs{w}}_{i^\prime}\}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_1} C_t W^{1, p}_{\bs{x}}}.
\label{contraction: F contraction expression}
\end{align}
Because of the condition (\ref{contraction: F cond 1}), the term depending on $i$ on the right-hand side of (\ref{contraction: F contraction expression}) is nonincreasing with $i$. Therefore, to make sure that the constant on the r.h.s. is less than $1$, we only need check for the case $i = 1$. We get two conditions:
\begin{align}
p < \frac{(\eta + \nu) d}{\eta d + 1 + \beta - \log_2(2^\beta - 1)},
\label{contraction: F cond 2}
\end{align}
and 
\begin{align}
\gamma_1 < \frac{\eta d}{p}  - \beta - \eta d.
\label{contraction: F cond 3}
\end{align}
From (\ref{contraction: F cond 1}) and (\ref{contraction: F cond 3}) existence of a feasible $\gamma_1$ then requires
\begin{align}
\nu \left(1 - \frac{d}{p}\right) < \frac{\eta d}{p}  - \beta - \eta d,
\end{align}
which implies
\begin{align}
p < \frac{(\eta + \nu) d}{\eta d + \nu + \beta} \qquad \implies \qquad \frac{\eta d + \nu + \beta}{(\eta + \nu) d} < \frac{1}{p}
\label{contraction: F main cond}
\end{align}
Once we satisfy (\ref{contraction: F main cond}), the condition (\ref{contraction: F cond 2}) is automatically satisfied if we choose $\nu > \nu_0 \coloneqq 1 - \log_2 (2^\beta - 1)$.

\subsection{Contraction for $G$}
We define a set of infinite sequences of scalar fields as
\begin{align}
\mathcal{Y} \coloneqq \Bigg\{ \{\varrho_i\}_{i \in \mathbb{N}} \in \ell^\infty_{\gamma_2}\left(\mathbb{N}; L^\infty([0, 1]; L^r(\mathbb{R}^d))\right) \cap  \ell^\infty_{\gamma_3}\left(\mathbb{N}; \text{Lip}([0, 1]; W^{1, -q}(\mathbb{R}^d))\right) \; \Bigg| \qquad \qquad \qquad \nonumber \\
\varrho_i(0, \cdot) = \rho^{in}_i, \; \varrho_i(1, \cdot) = \rho^{out}, \; \supp_{\bs{x}} \varrho_i(t, \cdot) \subseteq \left[-\frac{1}{2}, \frac{1}{2}\right]^d \Bigg\}
\end{align}
equip with the metric 
\begin{align}
\norm{\cdot}_{\ell^\infty_{\gamma_2} L^\infty_t L^r_{\bs{x}}} + \norm{\cdot}_{\ell^\infty_{\gamma_3} \text{Lip}_t W^{-1, q}_{\bs{x}}}
\end{align}
\noindent
Step 1 ($G : \mathcal{Y} \to \mathcal{Y}$): Let $\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}} \in \mathcal{Y}$, then from the definition of $G$ from \S \ref{sec: fixed-point mapping}, it is clear that 
\begin{enumerate}[label={(\roman*)}]
\item $G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(0, \cdot) = \rho^{in}_i$ after noting the fact that $2^{\nu d i} \rho_1(1, 2^{\eta + \nu i}(\bs{x} - \bs{c}_1)) = \rho^c_i(2^{\eta}(\bs{x} - \bs{c}_1))$,
\item $G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(1, \cdot) = \rho^{out}_i$,
\item $\supp_{\bs{x}} G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) \subseteq \left[-\frac{1}{2}, \frac{1}{2}\right]^d$.
\end{enumerate}
A few basic calculations show that for $k \in \{1, \dots 2^{\eta d}\}$, if $t \in \mathcal{T}^k_{(1)}$ then 
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} \leq \frac{k-1}{2^{\frac{\eta d}{r}}} \norm{\rho^{out}}_{L^r} + \frac{2^{\eta d}  - k}{2^{\frac{\eta d}{r}}} \norm{\rho^{c}_i}_{L^r} + 2^{\nu d i} \left(\frac{1}{2^{\eta + \nu i}} \right)^{\frac{d}{r}} \norm{\varrho_1}_{L^\infty_t L^r_{\bs{x}}}.
\end{align}
Noting that $\norm{\rho^{out}}_{L^r} \leq \norm{\rho^{c}_i}_{L^r}$ and that 
\begin{align}
\norm{\rho^{c}_i}_{L^r} = \left(2^{\nu d i} \right)^{\frac{r-1}{r}},
\end{align}
we get 
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} & \leq \left(2^{\eta d + \nu d i}\right)^{\frac{r-1}{r}} + 2^{\nu d i} \left(\frac{1}{2^{\eta + \nu i}} \right)^{\frac{d}{r}} \norm{\varrho_1}_{L^\infty_t L^r_{\bs{x}}} \nonumber \\
& \leq \left(2^{\eta d + \nu d i}\right)^{\frac{r-1}{r}} + 2^{\gamma_2 + \nu d i} \left(\frac{1}{2^{\eta + \nu i}} \right)^{\frac{d}{r}} \norm{\{\varrho_{i^\prime} \}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_2} L^\infty_t L^r_{\bs{x}}}.
\end{align}
Similarly for $t \in \mathcal{T}^k_{(2)}$, we get 
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} \leq \frac{k-1}{2^{\frac{\eta d}{r}}} \norm{\rho^{out}}_{L^r} + \frac{2^{\eta d}  - k}{2^{\frac{\eta d}{r}}} \norm{\rho^{c}_i}_{L^r} + 2^{\nu d i} \left(\frac{1}{2^{\eta + \nu i}} \right)^{\frac{d}{r}} + \frac{2^{\nu d (i+1)}}{2^{\frac{\eta d}{r}}} \norm{\ol{\rho}_b\left(\cdot, \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu (i+1)}}\right)}_{L^\infty_t L^r_{\bs{x}}},
\end{align}
which simplifies to 
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} \leq \left(2^{\eta d + \nu d i}\right)^{\frac{r-1}{r}} + 2^{\nu d i} \left(\frac{1}{2^{\eta + \nu (i+1)}} \right)^{\frac{d}{r}}.
\end{align}
For $t \in \mathcal{T}^k_{(3)}$, we get
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} \leq \left(2^{\eta d + \nu d i}\right)^{\frac{r-1}{r}} + \frac{1}{2^{\frac{\eta d}{r}}} \norm{\varrho_{i+1}}_{L^\infty_t L^r_{\bs{x}}} \leq \left(2^{\eta d + \nu d i}\right)^{\frac{r-1}{r}} + \frac{2^{\gamma_2(i+1)}}{2^{\frac{\eta d}{r}}} \norm{\{\varrho_{i^\prime} \}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_2} L^\infty_t L^r_{\bs{x}}}.
\end{align}
Finally, if $t = \tau^{2^{\eta d}}_{\infty}$, we have
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} = 1.
\end{align}
Combining everything gives
\begin{align}
\frac{1}{2^{\gamma_2 i}} \norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})}_{L^\infty_t L^r_{\bs{x}}} \; \lesssim_{d, r, \gamma_2, \eta, \nu} \; \sup_{i \in \mathbb{N}} \frac{\left(2^{\nu d i}\right)^{\frac{r-1}{r}}}{2^{\gamma_2 i}} \max \left\{1, \norm{\{\varrho_{i^\prime} \}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_2} L^\infty_t L^r_{\bs{x}}}\right\}.
\end{align}
Therefore, for the left-hand side to be bounded we need
\begin{align}
\frac{\nu d (r - 1)}{r} < \gamma_2.
\end{align}
Given two infinite sequences of scalar fields $\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}} \in \mathcal{Y}$ and $\{\varsigma_{i^\prime}\}_{i^\prime \in \mathbb{N}} \in \mathcal{Y}$, we find that 


For $t \in \mathcal{T}^k_{(1)}$, we have
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - G_i(\{\varsigma_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} \leq  2^{\gamma_2 + \nu d i} \left(\frac{1}{2^{\eta + \nu i}} \right)^{\frac{d}{r}} \norm{\{\varrho_{i^\prime} \}_{i^\prime \in \mathbb{N}} - \{\varsigma_{i^\prime} \}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_2} L^\infty_t L^r_{\bs{x}}}.
\end{align}
For $t \in \mathcal{T}^k_{(2)}$, we have
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - G_i(\{\varsigma_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} = 0.
\end{align}
For $t \in \mathcal{T}^k_{(3)}$, we have
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - G_i(\{\varsigma_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} = \frac{2^{\gamma_2(i+1)}}{2^{\frac{\eta d}{r}}} \norm{\{\varrho_{i^\prime} \}_{i^\prime \in \mathbb{N}} - \{\varsigma_{i^\prime} \}_{i^\prime \in \mathbb{N}}}_{\ell^\infty_{\gamma_2} L^\infty_t L^r_{\bs{x}}}.
\end{align}
Finally, if $t = \tau^{2^{\eta d}}_{\infty}$, we have
\begin{align}
\norm{G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) - G_i(\{\varsigma_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot)}_{L^r} = 0.
\end{align}
For $G$ to be a contraction, we need
\begin{align}
\sup_{i \in \mathbb{N}} \max\left\{\frac{2^{\nu d i}}{2^{\gamma_2 (i-1)}} \left(\frac{1}{2^{\eta + \nu i}} \right)^{\frac{d}{r}}, \frac{2^{\gamma_2}}{2^{\frac{\eta d}{r}}}\right\} < 1, 
\end{align}
which gives
\begin{align}
\gamma_2 < \frac{\eta d}{r}.
\end{align}
A feasible value of $\gamma_2$ then requires
\begin{align}
& r < \frac{\eta + \nu}{\nu} \nonumber \\
& \implies \frac{\nu}{\eta + \nu} < \frac{1}{r} \nonumber \\
& \implies \frac{\nu}{\eta + \nu}\frac{d-1}{d} < \frac{1}{r} \frac{d-1}{d} \nonumber \\
& \implies \frac{1}{r} \frac{1-d}{d} < \frac{\nu}{\eta + \nu}\frac{1-d}{d} \nonumber \\
& \implies  1 + \frac{1}{r} \frac{1-d}{d} < 1 + \frac{\nu}{\eta + \nu}\frac{1-d}{d} = \frac{\eta d + \nu}{\eta d + \nu d} < \frac{\eta d + \nu + \beta}{\eta d + \nu d} < \frac{1}{p} \nonumber \\
& \implies \boxed{1 + \frac{1}{r} \frac{1}{d} < \frac{1}{r} + \frac{1}{p}}
\end{align}

Next we show $G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})$ is Lipschitz in time in $W^{-1, q}$ topology and will obtain a bound on the $\text{Lip}_t W^{-1, q}_{\bs{x}}$-norm. We proceed in two steps: in the first step we show that $G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})$ is Lipschitz in time in the $W^{-1, q}$ topology in the interior of time intervals $\mathcal{T}^k_{(1)}$, $\mathcal{T}^k_{(2)}$ and $\mathcal{T}^k_{(3)}$. In the second step we show that $G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})$ is continuous in time in $W^{-1, q}$ topology at the interfaces $\tau^k_1$, $\tau^k_{mid}$, $\tau^k_2$ and $\tau^k_\infty$.

We start with the second step. 

Continuity at $t = \tau^k_1$: Substituting $t = \tau^k_1$ in the expression of $G_i$, we get
\begin{align}
G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(\tau^k_1, \cdot) = \sum_{1 \leq k^\prime < k} \rho^{out}(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \sum_{k < k^\prime \leq 2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + 2^{\nu d i} \varrho_1\left(1,  2^{\eta + \nu i}(\bs{x} - \bs{c}_k)\right).
\end{align}
Next, we can verify that 
\begin{align}
\varrho_1\left(1,  2^{\eta + \nu i}(\bs{x} - \bs{c}_k)\right) = \rho^c_i(2^\eta(\bs{x} - \bs{c}_k)),
\end{align}
which implies
\begin{align}
G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(\tau^k_1, \cdot) = \sum_{1 \leq k^\prime < k} \rho^{out}(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \sum_{k \leq k^\prime \leq 2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime})).
\end{align}
If $k = 1$, we see that $G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})$ is equal to the initial condition $\rho^{in}_i$. If $k \geq 2$ then check for the continuity from the left at $t = \tau^k_1$. We first see that 
\begin{align}
\varrho_{i+1}(1, 2^\eta(\bs{x} - \bs{c}_k)) = \rho^{out}(1, 2^\eta(\bs{x} - \bs{c}_k)).
\end{align}
This implies that
\begin{align}
G_i(\{\varrho_{i^\prime}\}_{i^\prime \in \mathbb{N}})(t, \cdot) \to  \sum_{1 \leq k^\prime < k} \rho^{out}(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \sum_{k \leq k^\prime \leq 2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime})) \quad \text{in} \quad W^{1, -q} \quad \text{as} \quad t \nearrow \tau^k_{1}.
\end{align}

Continuity at $t = \tau^k_{mid}$. We only need to show
\begin{align}
2^{\nu d i}\rho_{1}\left(0, 2^{\eta + \nu i}(\bs{x} - \bs{c}_k)\right) = 2^{\nu d (i + 1)} \ol{\rho}_b\left(0, 2^\eta (\bs{x} - \bs{c}_k); \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu(i+1)}}\right),
\end{align}
which requires us to show
\begin{align}
2^{\nu d i}\rho_{1}\left(0, 2^{\nu i}\bs{x}\right) = 2^{\nu d (i + 1)} \ol{\rho}_b\left(0, \bs{x}; \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu(i+1)}}\right),
\end{align}.
We see that
\begin{align}
2^{\nu d i}\rho_{1}\left(0, 2^{\nu i}\bs{x}\right) & = 2^{\nu d i} \rho^{in}_1(2^{\nu i} \bs{x}) \nonumber \\
& = \sum_{k^\prime = 1}^{2^{\eta d}} 2^{\nu d i} \rho^c_i(2^\eta(2^{\nu i} \bs{x} - \bs{c}_{k^\prime})) \nonumber \\
& = 
\begin{cases}
& 2^{\nu d (i + 1)} \quad \text{if} \quad 2^{\nu i} \bs{x} \in \bigcup\limits_{k^\prime \in \{1, \dots 2^{\eta d}\}} \ol{Q}\left(\frac{\bs{c}_{k^\prime}}{2^\eta}, \frac{1}{2^{\eta + \nu}}\right) \\
& 0 \qquad \text{otherwise}.
\end{cases} \nonumber \\
& = 
\begin{cases}
& 2^{\nu d (i + 1)} \quad \text{if} \quad \bs{x} \in \bigcup\limits_{k^\prime \in \{1, \dots 2^{\eta d}\}} \ol{Q}\left(\frac{\bs{c}_{k^\prime}}{2^{\eta + \nu i}}, \frac{1}{2^{\eta + \nu(i+1)}}\right) \\
& 0 \qquad \text{otherwise}.
\end{cases} \nonumber \\
& = 2^{\nu d (i + 1)} \ol{\rho}_b\left(0, \bs{x}; \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu(i+1)}}\right).
\end{align}
We now consider continuity at $t = \tau^k_2$. We need to show
\begin{align}
\rho_{i+1}(0, 2^{\eta}(\bs{x} - \bs{c}_k)) = 2^{\nu d (i + 1)} \ol{\rho}_b\left(1, 2^{\eta}(\bs{x} - \bs{c}_k); \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu(i+1)}}\right),
\end{align}
which requires us to show
\begin{align}
\rho_{i+1}(0, \bs{x}) = 2^{\nu d (i + 1)} \ol{\rho}_b\left(1, \bs{x}; \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu(i+1)}}\right),
\end{align}
We have that
\begin{align}
& \rho_{i+1}(0, \bs{x}) = \sum_{k^\prime = 1}^{2^{\eta d}}  \rho^c_{i+1}(2^\eta( \bs{x} - \bs{c}_{k^\prime})) \nonumber \\
& = 
\begin{cases}
& 2^{\nu d (i + 1)} \quad \text{if} \quad  \bs{x} \in \bigcup\limits_{k^\prime \in \{1, \dots 2^{\eta d}\}} \ol{Q}\left(\bs{c}_{k^\prime}, \frac{1}{2^{\eta + \nu i}}\right) \\
& 0 \qquad \text{otherwise}.
\end{cases} \nonumber \\
& = 2^{\nu d (i + 1)} \ol{\rho}_b\left(1, \bs{x}; \frac{1}{2^{\nu i}}, \frac{1}{2^{\nu(i+1)}}\right).
\end{align}

==> fixed_point_mapping.tex <==
\section{Fixed-point mapping}
\label{sec: fixed-point mapping}
As mentioned in the outline in section \ref{sec: outline}, our construction of the vector field and the corresponding solution of the continuity equation is based on the Banach fixed-point theorem applied to mappings $F$ and $G$. The goal of this section is to define these mappings $F$ and $G$. The function $F$ takes infinite sequence of vector fields $\{\bs{w}^{in}_i:[0,1] \times \mathbb{R}^d \to \mathbb{R}^d\}_{i \in \mathbb{N}}$ as an input and outputs an infinite sequence of vector fields $\{\bs{w}^{out}_i:[0,1] \times \mathbb{R}^d \to \mathbb{R}^d\}_{i \in \mathbb{N}}$:
\begin{align}
\{\bs{w}^{out}_i\}_{i \in \mathbb{N}} = F(\{\bs{w}^{in}_i\}_{i \in \mathbb{N}}).  
\end{align}
In the component form we write, $F = \{F_i\}_{i \in \mathbb{N}}$, where 
\begin{align}
\bs{w}^{out}_i = F_i(\{\bs{w}^{in}_i\}_{i \in \mathbb{N}}).   
\end{align}
Next, we specify these component mappings $F_i$. Let $\{\bs{w}_i:[0,1] \times \mathbb{R}^d \to \mathbb{R}^d\}_{i \in \mathbb{N}}$. For $k \in \{1, \dots 2^{\eta d}\}$ and $t \in \mathcal{T}^k_{(1)}$, we define
\begin{align}
F_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq 
\frac{1}{2^{\eta + \nu i}} \frac{1}{\tau^k_{mid} - \tau_1^k} \bs{w}_1 \left(\frac{\tau_{mid}^k - t}{\tau_{mid}^k - \tau^k_1},  2^{\eta + \nu i}(\bs{x} - \bs{c}_k)\right),
\end{align}
for $t \in \mathcal{T}^k_{(2)}$, we define
\begin{align}
F_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq 
\frac{1}{2^{\eta}} \frac{1}{\tau^k_{2} - \tau_{mid}^k} \ol{\bs{v}}_b \left(\frac{t + \tau_{mid}^k}{\tau_{2}^k - \tau^k_{mid}},  2^{\eta}(\bs{x} - \bs{c}_k); \frac{1}{2^{\eta + \nu i}}, \frac{1}{2^{\eta + \nu (i+1)}}\right),
\end{align}
for $t \in \mathcal{T}^k_{(3)}$, we define
\begin{align}
F_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq 
\frac{1}{2^{\eta}} \frac{1}{\tau^k_{\infty} - \tau_2^k} \bs{w}_{i+1} \left(\frac{t - \tau_{2}^k}{\tau_{\infty}^k - \tau^k_2},  2^{\eta}(\bs{x} - \bs{c}_k)\right),
\end{align}
and finally for $t = \tau^{2^{\eta d}}_{\infty}$, we define
\begin{align}
F_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq \bs{0}.
\end{align}
Notice that in the time interval $\mathcal{T}^k_{(2)}$, $F_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x})$ is defined as a rescaled copy of the building block vector field $\ol{\bs{v}}_b$ from section \ref{sec: building block}.

We now define the mapping $G$, which takes infinite sequence of scalar fields $\{\varrho^{in}_i:[0,1] \times \mathbb{R}^d \to \mathbb{R}\}_{i \in \mathbb{N}}$ as an input and outputs an infinite sequence of scalar fields $\{\varrho^{out}_i:[0,1] \times \mathbb{R}^d \to \mathbb{R}\}_{i \in \mathbb{N}}$. In a similar way as before, we define $G_i$, the $i$th component of $G$, on different time intervals. For $k \in \{1, \dots 2^{\eta d}\}$ and $t \in \mathcal{T}^k_{(1)}$, we define
\begin{align}
G_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq \sum_{1 \leq k^\prime < k} \rho^{out}(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \sum_{k < k^\prime \leq 2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + 2^{\nu d i} \rho_1\left(\frac{\tau_{mid}^k - t}{\tau_{mid}^k - \tau^k_1},  2^{\eta + \nu i}(\bs{x} - \bs{c}_k)\right),
\end{align}
for $t \in \mathcal{T}^k_{(2)}$, we define
\begin{align}
G_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq \sum_{1 \leq k^\prime < k} \rho^{out}(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \sum_{k < k^\prime \leq 2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime})) \qquad \qquad \\
+ \; 2^{\nu d (i+1)} \ol{\rho}_b \left(\frac{t + \tau_{mid}^k}{\tau_{2}^k - \tau^k_{mid}},  2^{\eta}(\bs{x} - \bs{c}_k); \frac{1}{2^{\eta + \nu i}}, \frac{1}{2^{\eta + \nu (i+1)}}\right),
\end{align}
for $t \in \mathcal{T}^k_{(3)}$, we define
\begin{align}
G_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq \sum_{1 \leq k^\prime < k} \rho^{out}(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \sum_{k < k^\prime \leq 2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime})) + \rho_{i+1}\left(\frac{ t - \tau_{2}^k}{\tau_{\infty}^k - \tau^k_2},  2^{\eta}(\bs{x} - \bs{c}_k)\right),
\end{align}
and finally for $t = \tau^{2^{\eta d}}_{\infty}$, we define
\begin{align}
G_i(\{\bs{w}_i\}_{i \in \mathbb{N}})(t, \bs{x}) \coloneqq \rho^{out}(\bs{x}).
\end{align}
The goal of the next section is to show that the mapping $F$ and $G$ have unique fixed points in appropriate functional spaces and the fixed points solves the continuity equation.

==> notations.tex <==
\section{Notations}
\label{notation}

{\color{blue}EB: I'm going to eliminate this section. I propose to introduce the various notations when they get used for the first time } \\
{\color{violet}AK: I agree. Once we have moved these notations to relevant places, we can remove this section.}

\noindent
\textbf{Notation 1} (\textit{General})
A cube \\
Domain of interest $\mathscr{D} \coloneqq \left[-\frac{1}{2}, \frac{1}{2}\right]^d$
\\
\\
\textbf{Notation 2} (\textit{Parameters})
Our construction of the vector field involves three free parameters:
\begin{enumerate}[label=(\roman*)]
  \item $\beta \in (0, 1)$, involved in the definition of time series,
  \item $ 0 < \nu$, governing the size of cubes in the construction
  \item $\eta \in \mathbb{N}$, governing the number of cubes.
\end{enumerate}
We will achieve the desired range of exponents as stated in Theorem \ref{Intro: main thm} by adjusting the values of these parameters. 
\\
\\
% \textbf{Notation 3} (\textit{Time series})
% In our vector field construction, we work on the time interval $[0, 1]$. Given parameters $0 < \beta < 1$ and $\eta \in \mathbb{N}$, we define useful checkpoints. For $k \in \{1, \dots 2^{\eta d}\}$, we define 
% \begin{align}
% & \tau^k_1 \coloneqq \frac{(k-1)}{2^{\eta d}}, \nonumber \\
% & \tau^k_2 \coloneqq \left(k - \frac{1}{2^\beta}\right) \frac{1}{2^{\eta d}}, \nonumber \\ 
% & \tau^k_{mid} \coloneqq \frac{\tau^k_1 + \tau^k_2}{2}, \nonumber \\
% & \tau^k_\infty = \frac{k}{2^{\eta d}}.
% \end{align}
% With the definition of checkpoints above, it is clear that for every $k \in \{1, \dots 2^{\eta d}\}$
% \begin{align}
% \tau^k_2 - \tau^k_1 = \frac{2^\beta - 1}{2^\beta} \frac{1}{2^{\eta d}} \quad 
% \text{and} \quad
% \tau^k_{\infty} - \tau^k_{2} = \frac{1}{2^\beta} \frac{1}{2^{\eta d}}
% \end{align}
% and for every $k \in \{1, \dots 2^{\eta d} - 1\}$
% \begin{align}
% \tau^{k+1}_1 = \tau^k_{\infty}.
% \end{align}
% With the help of these checkpoints, for $k \in \{1, \dots 2^{\eta d}\}$, we define a time interval as
% \begin{align}
% \mathcal{T}^k \coloneqq [\tau_1^k, \tau_{\infty}^k),
% \end{align}
% which is further divided into three time intervals as
% \begin{align}
% \mathcal{T}_{(1)}^k \coloneqq [\tau_1^k, \tau_{mid}^k], \qquad \mathcal{T}_{(2)}^k \coloneqq (\tau_{mid}^k, \tau_{2}^k), \quad
% \text{and} \quad 
% \mathcal{T}_{(3)}^k \coloneqq [\tau_2^k, \tau_{\infty}^k].
% \end{align}
% \\
% \\



% \textbf{Notation 4} (\textit{A few points in} $\mathscr{D}$)
% Given an integer $k \in \{1, 2, \dots 2^{\eta d}\}$, we define $(j_1^k, \dots j_d^k) \in \{0, \dots 2^\eta - 1\}^d$, a $d$-tuple of integers, such that
% \begin{align}
% 1 + \sum_{i = 1}^d 2^{\eta (i-1)} j_i^k = k.
% \end{align}
% It is clear that there is a unique such $d$-tuple. For a given $k \in \{1, 2, \dots 2^{\eta d}\}$, we define $c_k \in \left[-\frac{1}{2}, \frac{1}{2}\right]^d$ as
% \begin{align}
% c_k \coloneqq \left(\frac{1}{2^\eta} \left[j_1^k - \frac{2^\eta - 1}{2}\right], \dots \frac{1}{2^\eta} \left[j_d^k - \frac{2^\eta - 1}{2}\right]\right).
% \end{align}
% For given $0 < a < 1$, we also define
% \begin{align}
% d_k^a \coloneqq \left(\frac{a}{2^\eta} \left[j_1^k - \frac{2^\eta - 1}{2}\right], \dots \frac{a}{2^\eta} \left[j_d^k - \frac{2^\eta - 1}{2}\right]\right).
% \end{align}
% \\
% \\





% \textbf{Notation 5} (\textit{Initial and final density fields}) The construction of the required vector field $\bs{v}$ and a corresponding solution $\rho$ of the continuity equations will be a based on a fixed point iteration applied to an infinite sequence of vector fields $\{\bs{v}_i\}_{i \in \mathbb{N}}$ and corresponding solutions $\{\rho_i\}_{i \in \mathbb{N}}$. Here, we define the different initial and final conditions these solutions $\rho_i$ will satisfy. We first define $\rho^{out} : \mathbb{R}^d \to \mathbb{R}$ as 
% \begin{align}
% \rho^{out} \coloneqq 
% \begin{cases}
% & 1 \quad \text{if} \quad \bs{x} \in \ol{Q}(0, 1), \\
% & 0 \quad \text{otherwise}.
% \end{cases}
% \end{align}
% Next, for every $i \in \mathbb{N}$, we define 
% \begin{align}
% \rho^{c}_i \coloneqq 
% \begin{cases}
% & 2^{\nu d i} \quad \text{if} \quad \bs{x} \in \ol{Q}(0,  \frac{1}{2^{\nu i}}), \\
% & 0 \quad \text{otherwise},
% \end{cases}
% \end{align}
% Using which we define
% \begin{align}
% \rho^{in}_i \coloneqq \sum_{k^\prime = 1}^{2^{\eta d}} \rho^{c}_i(2^\eta(\bs{x} - \bs{c}_{k^\prime}))  
% \end{align}
% For the $i$th problem the initial density is $\rho^{in}_i$ and the final density is $\rho^{out}$.



% \textbf{Notation 5} (\textit{Functional spaces}) 
% (i) $C([0, T]; W^{1, p})$ \\
% (ii) $L^\infty L^r$ \\
% (iii) We say a function $f \in W^{-1, q}(\mathbb{R}^d)$ if the norm $\norm{f}_{W^{-1, q}}$ defined as 
% \begin{align}
% \norm{f}_{W^{-1, q}} \coloneqq   \sup\limits_{\substack{\phi \in W^{1, q^\prime}_0 \\ \norm{\nabla \phi}_{L^{q^\prime}} \leq 1}} \int_{\mathbb{R}^d} f \phi \; {\rm d} \bs{x}.
% \end{align}
% is bounded. \\



% (iv) Given $\gamma \in \mathbb{R}$, we define $\ell^{\infty}_\gamma(\mathbb{N})$ to be the weighted version of $\ell^{\infty}(\mathbb{N})$ space. We say a sequence $\{a_i\}_{i \in \mathbb{N}} \in \ell^{\infty}_\gamma(\mathbb{N})$ if the norm 
% \begin{align}
% \norm{\{a_i\}_{i \in \mathbb{N}}}_{\ell^{\infty}_\gamma} \coloneqq \sup_{i \in \mathbb{N}} \frac{|a_i|}{2^{\gamma i}}
% \end{align}
% is bounded.

==> r_1.tex <==
\section{Nonuniqueness in $L^r$}
\label{sec:r>1}



To achieve nonunique solutions to the transport equation with density in $L^r$, we introduce a variant of the previous construction.

Given parameters $\nu >0$ and $\eta \in \mathbb{N}$, governing the size and number of cubes respectively, we look for a velocity field $u$ that acts as shown in the picture below.


\begin{figure}[h]
\centering
 \includegraphics[scale = 0.4]{Figures/Original_problem.eps}
 \caption{shows the initial and final density. The intensity of the red color indicates the magnitude of the density. $\nu = 2/3$, $\eta = 2$, $d = 2$.}
 \label{fig: org prb}
\end{figure}



\subsection{Fixed point argument}

{
\color{blue}

Here we explain the fixed point argument, which is similar to the one for the $L^1$ case.


Most important point: We have to discuss carefully the parameters and explain that we get the same range as in the convex integration. 
\begin{equation}
    \frac{1}{p} + \frac{1}{r} > 1 + \frac{1}{d}
\end{equation}

} 
